Asteroid-Meteoroid Complexes

This is an overview of recent research on meteors and the parent bodies from which they are produced. While many meteor showers result from material ejected by comets, two out of the three strongest annual showers (the Geminids and the Quadrantids) are associated with objects whose physical properties are apparently those of asteroids. In the last decades dynamical and observational studies have confirmed the existence of a number of Asteroid-Meteoroid Complexes, comprising streams and several macroscopic, split fragments. Spectroscopy of meteor showers has been utilized to investigate the perihelion-dependent thermal alteration while in interplanetary space. In this chapter, we review characteristics of the complexes, including those of some minor streams. The scientific interest is to trace the physical and dynamical properties of the complexes back to the evolutionary pathways to learn about the variety of production processes of meteoroids to form streams. We also discuss open questions in the field for the next decade.

==> authors.tex <==
\contributor{Toshihiro Kasuga}
{Public Relations Center\\
National Astronomical Observatory of Japan\\
2-21-1 Osawa \\
Mitaka, Tokyo 181-8588\\
Japan}
{Department of Physics\\
Kyoto Sangyo University\\
Motoyama, Kamigamo Kita-ku\\ 
Kyoto 603-8555, Japan
}
\contributor{David Jewitt}
{Earth, Planetary and Space Sciences / Physics and Astronomy \\
University of California at Los Angeles \\
595 Charles Young Drive East Los Angeles, CA 90095-1567 \\
USA}


==> editedloc.tex <==
\contentsline {contrib}{{\scshape toshihiro kasuga}\\
{Public Relations Center\\
National Astronomical Observatory of Japan\\
2-21-1 Osawa Mitaka\\
Tokyo 181-8588 \\ Japan \\ \\
Department of Physics\\
Kyoto Sangyo University \\
Motoyama, Kamigamo Kita-ku \\
Kyoto 603-8555 \\ Japan }}{2}
%
\contentsline {contrib}{{\scshape david jewitt}\\
{Earth, Planetary and Space Sciences / Physics and Astronomy \\ 
University of California at Los Angeles\\ 
595 Charles Young Drive East Los Angeles\\ 
CA 90095-1567 \\ 
USA}}{2}


